Learning Deep Semantics for Test Completion

Writing tests is a time-consuming yet essential task during software development. We propose to leverage recent advances in deep learning for text and code generation to assist developers in writing tests. We formalize the novel task of test completion to automatically complete the next statement in a test method based on the context of prior statements and the code under test. We develop TeCo -- a deep learning model using code semantics for test completion. The key insight underlying TeCo is that predicting the next statement in a test method requires reasoning about code execution, which is hard to do with only syntax-level data that existing code completion models use. TeCo extracts and uses six kinds of code semantics data, including the execution result of prior statements and the execution context of the test method. To provide a testbed for this new task, as well as to evaluate TeCo, we collect a corpus of 130,934 test methods from 1,270 open-source Java projects. Our results show that TeCo achieves an exact-match accuracy of 18, which is 29% higher than the best baseline using syntax-level data only. When measuring functional correctness of generated next statement, TeCo can generate runnable code in 29% of the cases compared to 18% obtained by the best baseline. Moreover, TeCo is significantly better than prior work on test oracle generation.

==> defs/defs-code.tex <==
%%% defs-code.tex
%%% Utility Commands for Code Listings
%%% Version 1.0.2

%%%==========
%%% COPIED FROM vkuncak/doc/vmcai09/defs.tex
\definecolor{gray}{RGB}{211,211,211}
\newcommand{\jbasicstyle}{\small\sffamily} % Style of code
\newcommand{\textcode}[1]{{#1}}
\newcommand{\jnumberstyle}{\scriptsize}
\newcommand{\Hilight}{\makebox[0pt][l]{\color{gray}\rule[-3pt]{0.80\linewidth}{9pt}}}

\lstdefinelanguage{pseudo}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=left, % none for no numbers
  numberstyle=\jnumberstyle,
  numbersep=4pt,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=10pt,
%  mathescape=false,
}

\lstdefinelanguage{todo-comment}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=none,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=-10pt,
%  mathescape=false,
}

\lstdefinelanguage{java-pretty}
{
  language=java,
  numbers=left,
  numbersep=4pt,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=16pt,
  showstringspaces=false,
}

\lstdefinelanguage{java-pretty-no-number}
{
  language=java,
  numbers=none,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=0,
  showstringspaces=false,
}
\lstset{escapeinside={(*@}{@*)}}

%%%==========


==> defs/defs-logic.tex <==
%%% defs-logic.tex
%%% Utility Commands for Logic Symbols
%%% Version 1.1.0

%%% Basic Logic
% True & False
\newcommand{\ltrue}{\top} % ⊤
\newcommand{\lfalse}{\bot} % ⊥

% Operators
% \land ∧
% \lor ∨
% \lnot ¬
\newcommand{\limply}{\rightarrow} % →
\newcommand{\liff}{\leftrightarrow} % ↔
\newcommand{\lcofactor}{\downarrow} % ↓

\newcommand{\llimply}{\Rightarrow} % ⇒
\newcommand{\lliff}{\Leftrightarrow} % ⇔
\newcommand{\lsat}{\vDash} % ⊨
\newcommand{\lnsat}{\nvDash} % ⊭

% Quantifiers
\newcommand{\lqall}[1]{\forall #1.~} % ∀x.
\newcommand{\lqexist}[1]{\exists #1.~} % ∃x.
\newcommand{\lqallOnly}[1]{\forall #1 } % ∀x
\newcommand{\lqexistOnly}[1]{\exists #1 } % ∃x

% Big Operators
\newcommand{\lAnd}[1]{\bigwedge_{\substack{#1}}} % ⋀
\newcommand{\lOr}[1]{\bigvee_{\substack{#1}}} % ⋁

%%% Set
\newcommand{\set}[1]{\{#1\}} % {x, y, z}
\newcommand{\Set}[1]{\left\{#1\right\}} % \left{ x, y, z \right}
\newcommand{\tuple}[1]{\langle#1\rangle} % <a, b, c>
\newcommand{\Tuple}[1]{\left\langle#1\right\rangle} % \left< a, b, c \right>

\newcommand{\sunion}{\cup} % ∪
\newcommand{\sinter}{\cap} % ∩


==> figs/semdata-example.tex <==
% public class GMOperation {
%   public GMOperation addImage(final File file) {
%     if (file == null) {
%       throw new IllegalArgumentException(
%         "file must be defined");
%     }
%     getCmdArgs().add(file.getPath());
%     return this; 
%   }
% ... }

% public class GMOperationTest {
%   GMOperation sut;
%   @Before
%   public void setup() {... sut = new GMOperation(); ...}

%   @Test 
%   public void addImage_ThrowsException_WhenFileIsNull() 
%       throws Exception {
%     exception.except(IllegalArgumentException.class);
%     sut.addImage((File) null);
%   }
% ... }


\newsavebox{\lstExampleFull}
\begin{lrbox}{\lstExampleFull}
\begin{lstlisting}[language=java-pretty]
public class GMOperation 
    extends org.im4java.core.GMOperation {
  public GMOperation addImage(final File file) {...}(*@\label{line:mut-sign}@*)
...}

public class GMOperationTest {
  GMOperation sut;(*@\label{line:field-sut}@*)
  @Before 
  public void setup() {... sut = new GMOperation(); ...}(*@\label{line:setup}@*)

  @Test 
  public void addImage_ThrowsException_WhenFileIsNull()
      throws Exception {
    exception.except(IllegalArgumentException.class);
    sut.addImage((File) null);(*@\label{line:next-stmt}@*)
  }
...}
\end{lstlisting}
\end{lrbox}

\begin{tikzpicture}[
  font=\footnotesize, 
  box/.style={rectangle, scale=1, inner sep=1pt},
  box-bg/.style={box},
  box-label/.style={box, inner sep=2pt, draw=none, fill=blue!10, rounded corners},
  color-suf/.style={draw=yellow!80!black, fill=yellow!10},
  color-sem/.style={draw=blue!80!black, fill=blue!10},
  color-output/.style={draw=green!80!black, fill=green!10},
  anno/.style={font={\footnotesize}},
]
  \node (c-nw) at (0,0) [coordinate] {};

  \node (bg-s2) [below right = 4ex and 14.85em of c-nw] [box-bg, color-sem, minimum height=2ex, minimum width=2em] {};
  \node (l-s2) [below right = .1ex and 0 of bg-s2.south west] [box-label] {(\UseMacro{no-types-absent})~\UseMacro{name-types-absent}};
  \node (bg-s4) [below right = 13ex and .65em of c-nw] [box-bg, color-sem, minimum height=4ex, minimum width=23em] {};
  \node (l-s4) [below left = .1ex and 0 of bg-s4.south east] [box-label] {(\UseMacro{no-setup-teardown})~\UseMacro{name-setup-teardown}};
  \node (bg-output) [below right = 25.5ex and 1.35em of c-nw] [box-bg, color-output, minimum height=2ex, minimum width=11em] {};
  \node (b-full) [below right = 0 and 0 of c-nw] [box] {\usebox\lstExampleFull};

\end{tikzpicture}


==> tables/table-corpus.tex <==

%% Automatically generated by pyutil.latex 

\begin{tabular}{@{}l|r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{}}
\toprule
 & \textbf{\UseMacro{TH-num_proj}} & \textbf{\UseMacro{TH-num_test}} & \textbf{\UseMacro{TH-num_stmt}} & \textbf{\UseMacro{TH-tok_test}} & \textbf{\UseMacro{TH-tok_mut}} \\ 
\midrule
\UseMacro{TH-corpus-all}
 & \UseMacro{corpus-all-num_proj}
 & \UseMacro{corpus-all-num_test}
 & \UseMacro{corpus-all-num_stmt}
 & \UseMacro{corpus-all-tok_test}
 & \UseMacro{corpus-all-tok_mut}
\\
\UseMacro{TH-corpus-train}
 & \UseMacro{corpus-train-num_proj}
 & \UseMacro{corpus-train-num_test}
 & \UseMacro{corpus-train-num_stmt}
 & \UseMacro{corpus-train-tok_test}
 & \UseMacro{corpus-train-tok_mut}
\\
\UseMacro{TH-corpus-val}
 & \UseMacro{corpus-val-num_proj}
 & \UseMacro{corpus-val-num_test}
 & \UseMacro{corpus-val-num_stmt}
 & \UseMacro{corpus-val-tok_test}
 & \UseMacro{corpus-val-tok_mut}
\\
\UseMacro{TH-corpus-test}
 & \UseMacro{corpus-test-num_proj}
 & \UseMacro{corpus-test-num_test}
 & \UseMacro{corpus-test-num_stmt}
 & \UseMacro{corpus-test-tok_test}
 & \UseMacro{corpus-test-tok_mut}
\\
\bottomrule
\end{tabular}


==> tables/table-results-single-runnable-any-CSNm-bs.tex <==

%% Automatically generated by pyutil.latex 

\begin{tabular}{@{}l|@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{}}
\toprule
\textbf{\UseMacro{TH-model}}
 & \textbf{\UseMacro{TH-compilable}}
 & \textbf{\UseMacro{TH-runnable}}
 & \textbf{\UseMacro{TH-xmatch}}
 & \textbf{\UseMacro{TH-xmatch-top10}}
 & \textbf{\UseMacro{TH-bleu}}
 & \textbf{\UseMacro{TH-code-bleu}}
 & \textbf{\UseMacro{TH-edit-sim}}
 & \textbf{\UseMacro{TH-rouge}}
\\
\midrule
\UseMacro{model-codet5}
 & \textbf{\UseMacro{res-codet5-CSNm-eval-runnable-any-stmt/test-bs10-last-compilable}}
 & \textbf{\UseMacro{res-codet5-CSNm-eval-runnable-any-stmt/test-bs10-last-runnable}}
 & \UseMacro{res-codet5-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-codet5-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch-top10}
 & \UseMacro{res-codet5-CSNm-eval-runnable-any-stmt/test-bs10-last-bleu}
 & \UseMacro{res-codet5-CSNm-eval-runnable-any-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-codet5-CSNm-eval-runnable-any-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-codet5-CSNm-eval-runnable-any-stmt/test-bs10-last-rouge-f}
\\
\midrule
\UseMacro{model-teco-s1}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-any-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-any-stmt/test-bs10-last-runnable}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch-top10}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-any-stmt/test-bs10-last-bleu}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-any-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-any-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-any-stmt/test-bs10-last-rouge-f}
\\
\UseMacro{model-teco-s2}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-any-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-any-stmt/test-bs10-last-runnable}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch-top10}
 & \textbf{\UseMacro{res-teco-s2-CSNm-eval-runnable-any-stmt/test-bs10-last-bleu}}
 & \textbf{\UseMacro{res-teco-s2-CSNm-eval-runnable-any-stmt/test-bs10-last-code-bleu}}
 & \textbf{\UseMacro{res-teco-s2-CSNm-eval-runnable-any-stmt/test-bs10-last-edit-sim}}
 & \textbf{\UseMacro{res-teco-s2-CSNm-eval-runnable-any-stmt/test-bs10-last-rouge-f}}
\\
\UseMacro{model-teco-s3}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-any-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-any-stmt/test-bs10-last-runnable}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch-top10}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-any-stmt/test-bs10-last-bleu}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-any-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-any-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-any-stmt/test-bs10-last-rouge-f}
\\
\UseMacro{model-teco-s4}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-any-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-any-stmt/test-bs10-last-runnable}
 & \textbf{\UseMacro{res-teco-s4-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch}}
 & \textbf{\UseMacro{res-teco-s4-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch-top10}}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-any-stmt/test-bs10-last-bleu}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-any-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-any-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-any-stmt/test-bs10-last-rouge-f}
\\
\UseMacro{model-teco-s5}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-any-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-any-stmt/test-bs10-last-runnable}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch-top10}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-any-stmt/test-bs10-last-bleu}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-any-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-any-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-any-stmt/test-bs10-last-rouge-f}
\\
\UseMacro{model-teco-s6}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-any-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-any-stmt/test-bs10-last-runnable}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-any-stmt/test-bs10-last-xmatch-top10}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-any-stmt/test-bs10-last-bleu}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-any-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-any-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-any-stmt/test-bs10-last-rouge-f}
\\
\bottomrule
\end{tabular}


==> tables/table-results-single-runnable-assert-CSNm-bs.tex <==

%% Automatically generated by pyutil.latex 

\begin{tabular}{@{}l|@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{\hspace{2pt}}r@{}}
\toprule
\textbf{\UseMacro{TH-model}}
 & \textbf{\UseMacro{TH-compilable}}
 & \textbf{\UseMacro{TH-runnable}}
 & \textbf{\UseMacro{TH-xmatch}}
 & \textbf{\UseMacro{TH-xmatch-top10}}
 & \textbf{\UseMacro{TH-bleu}}
 & \textbf{\UseMacro{TH-code-bleu}}
 & \textbf{\UseMacro{TH-edit-sim}}
 & \textbf{\UseMacro{TH-rouge}}
\\
\midrule
\UseMacro{model-codet5}
 & \textbf{\UseMacro{res-codet5-CSNm-eval-runnable-assert-stmt/test-bs10-last-compilable}}
 & \textbf{\UseMacro{res-codet5-CSNm-eval-runnable-assert-stmt/test-bs10-last-runnable}}
 & \UseMacro{res-codet5-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-codet5-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch-top10}
 & \UseMacro{res-codet5-CSNm-eval-runnable-assert-stmt/test-bs10-last-bleu}
 & \UseMacro{res-codet5-CSNm-eval-runnable-assert-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-codet5-CSNm-eval-runnable-assert-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-codet5-CSNm-eval-runnable-assert-stmt/test-bs10-last-rouge-f}
\\
\midrule
\UseMacro{model-teco-s1}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-assert-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-assert-stmt/test-bs10-last-runnable}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch-top10}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-assert-stmt/test-bs10-last-bleu}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-assert-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-assert-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-teco-s1-CSNm-eval-runnable-assert-stmt/test-bs10-last-rouge-f}
\\
\UseMacro{model-teco-s2}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-assert-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-assert-stmt/test-bs10-last-runnable}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch-top10}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-assert-stmt/test-bs10-last-bleu}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-assert-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-assert-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-teco-s2-CSNm-eval-runnable-assert-stmt/test-bs10-last-rouge-f}
\\
\UseMacro{model-teco-s3}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-assert-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-assert-stmt/test-bs10-last-runnable}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-teco-s3-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch-top10}
 & \textbf{\UseMacro{res-teco-s3-CSNm-eval-runnable-assert-stmt/test-bs10-last-bleu}}
 & \textbf{\UseMacro{res-teco-s3-CSNm-eval-runnable-assert-stmt/test-bs10-last-code-bleu}}
 & \textbf{\UseMacro{res-teco-s3-CSNm-eval-runnable-assert-stmt/test-bs10-last-edit-sim}}
 & \textbf{\UseMacro{res-teco-s3-CSNm-eval-runnable-assert-stmt/test-bs10-last-rouge-f}}
\\
\UseMacro{model-teco-s4}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-assert-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-assert-stmt/test-bs10-last-runnable}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch-top10}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-assert-stmt/test-bs10-last-bleu}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-assert-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-assert-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-teco-s4-CSNm-eval-runnable-assert-stmt/test-bs10-last-rouge-f}
\\
\UseMacro{model-teco-s5}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-assert-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-assert-stmt/test-bs10-last-runnable}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch-top10}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-assert-stmt/test-bs10-last-bleu}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-assert-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-assert-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-teco-s5-CSNm-eval-runnable-assert-stmt/test-bs10-last-rouge-f}
\\
\UseMacro{model-teco-s6}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-assert-stmt/test-bs10-last-compilable}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-assert-stmt/test-bs10-last-runnable}
 & \textbf{\UseMacro{res-teco-s6-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch}}
 & \textbf{\UseMacro{res-teco-s6-CSNm-eval-runnable-assert-stmt/test-bs10-last-xmatch-top10}}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-assert-stmt/test-bs10-last-bleu}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-assert-stmt/test-bs10-last-code-bleu}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-assert-stmt/test-bs10-last-edit-sim}
 & \UseMacro{res-teco-s6-CSNm-eval-runnable-assert-stmt/test-bs10-last-rouge-f}
\\
\bottomrule
\end{tabular}

